Efficient Learning of Safe Driving Policy via Human-AI Copilot Optimization

Human intervention is an effective way to inject human knowledge into the training loop of reinforcement learning, which can bring fast learning and ensured training safety. Given the very limited budget of human intervention, it remains challenging to design when and how human expert interacts with the learning agent in the training. In this work, we develop a novel human-in-the-loop learning method called Human-AI Copilot Optimization (HACO).To allow the agent's sufficient exploration in the risky environments while ensuring the training safety, the human expert can take over the control and demonstrate how to avoid probably dangerous situations or trivial behaviors. The proposed HACO then effectively utilizes the data both from the trial-and-error exploration and human's partial demonstration to train a high-performing agent. HACO extracts proxy state-action values from partial human demonstration and optimizes the agent to improve the proxy values meanwhile reduce the human interventions. The experiments show that HACO achieves a substantially high sample efficiency in the safe driving benchmark. HACO can train agents to drive in unseen traffic scenarios with a handful of human intervention budget and achieve high safety and generalizability, outperforming both reinforcement learning and imitation learning baselines with a large margin. Code and demo videos are available at: https://decisionforce.github.io/HACO/.

==> figs/TMP-delete-this.tex <==

\section{Main Conclusion}

\section{Proof of Main Theorem}

In this section, we derive the upper bound of the discounted probability of failure of EGPO, showing that we can bound the training safety with the guardian.

\textit{\textbf{Notations.}}
Before starting, we firstly recap and describe the notations.
The switch function used in this work is:
\begin{equation}
    \mathcal T (s, a, \mathcal{E}) = (\hat{a}, \hat{c}) =
    \begin{cases}
      (a^E \sim \mathcal{E}(\cdot|s), 1), & \text{if } a \in \mathcal A_\eta(s) \\
      (a, 0), & \text{otherwise.}
    \end{cases}
\end{equation}
Therefore, at a given state, we can split the action space into two parts: where intervention will happen or will not happen if we sample action in it. 
We denote the \textit{confident action space} as $\mathcal A_\eta(s) = \{a: \mathcal E(a|s) \ge \eta \}$, which is related to the expert as well as $\eta$.
We also define the ground-truth indicator $C$ denoting whether the action will lead to unsafe state. This unsafe state is determined by the environment and is not revealed to learning algorithm:
\begin{equation}
C (s, a) = 
\begin{cases}
  1, & \text{if }s' = \mathcal P(s'|s, a) \text{ is an unsafe state,}
%  s' \notin \mathcal S_{\text{safe}},
%  s' = \mathcal P(s'|s, a) 
  \\
  0, & \text{otherwise.}
\end{cases}
\end{equation}

Therefore, at a given state $s$ the step-wise probability of failure for arbitrary policy $\pi$ is $\expect_{a\sim \pi(\cdot|s)} C(s, a) \in [0, 1]$.


Now we denote the \textit{cumulative discounted probability of failure} as $V^{\pi}(s_t) = \expect_{\pi} \sum_{t'=t}\gamma^{t'-t} I(s_{t'}, a_{t'})$, counting for the chance of entering dangerous states in current time step as well as in future trajectories deduced by the policy $\pi$.
We use $V^{\mathcal{E}} = \expect_{\tau\sim \mathcal{E}} V^{\mathcal{E}}(s_0)$ to denote the expected cumulative discounted probability of failure of the expert $\mathcal{E}$.

For simplicity, we can consider the actions post-processed by the guardian mechanism during training are sampled from a mixed policy $\hat{\pi}$, whose action probability can be written as:
\begin{equation}
\begin{aligned}
  \hat{\pi_\theta}(a|s) 
  & = 
  {\pi_\theta}(a|s) \mathbf 1_{a \in \mathcal A_\eta(s)}
  +
  \mathcal{E}(a|s)
  \mathop{\int}_{a'\notin \mathcal A_\eta(s)}
  {\pi_\theta}(a'|s) da' ~\\
  & = 
  {\pi_\theta}(a|s) \mathbf 1_{a \in \mathcal A_\eta(s)}
  +
  \mathcal{E}(a|s)F(s).
\end{aligned}
\end{equation}

Here the second term captures the situation that the learning agent takes arbitrary action $a'$ that triggers the expert to take over and chooses the action $a$. 
For simplicity, we use a shorthand
$F(s) = \mathop{\int}_{a'\notin \mathcal A_\eta(s)}  {\pi_\theta}(a'|s) da'$
.

Following the same definition as $V^{\mathcal{E}}$, we can also write the expected cumulative discounted probability of failure of the behavior policy as: $\hat{V} = \expect_{\tau\sim \hat{\pi}} \hat{V}(s_0)=\expect_{\hat{\pi}} \sum_{t=0}\gamma^{t} I(s_{t}, a_{t})$.

\textit{\textbf{Assumption.}}
Now we introduce one important assumption on the expert.

\begin{assumption}
\label{assumption:expert-failure-rate}
	For all states, the step-wise probability of expert producing unsafe action is bounded by a small value $\epsilon < 1$:
\begin{equation}
	\expect_{a\sim \mathcal E(\cdot|s)} I(s, a) \le \epsilon  .
\end{equation}
\end{assumption}

This assumption does not impose any constrain on the structure of the expert policy.


\textit{\textbf{Lemmas.}}
We propose several useful lemmas and the correspondent proofs, which are used in the main theorem.
\begin{lemma}[The performance difference lemma]
\label{lemma:performance-difference-lemma}
\begin{equation}
\hat{V} 
= 
V^{\mathcal{E}} + 
\cfrac{1}{1-\gamma}
\ \expect_{s\sim P_{\hat{\pi}}} \ 
\expect_{a\sim \hat{\pi}} \ 
[ A^{\mathcal E}(s, a) ].
\end{equation}
\end{lemma}

Here the $P_{\hat{\pi}}$ means the states are subject to the marginal state distribution deduced by the behavior policy $\hat{\pi}$. $A^{\mathcal E}(s, a)$ is the advantage of the expert in current state action pair: $A^{\mathcal E}(s, a) = I(s, a) + \gamma V^{\mathcal{E}}(s') - V^{\mathcal{E}}(s)$ and $s' = \mathcal P(s, a)$ is the next state.
This lemma is proposed and proved by \citet{kakade2002approximately} and is useful to show the behavior policy's safety.
In the original proposition, the $V$ and $A$ represents the expected discounted return and advantage w.r.t. the reward, respectively. However, we replace the reward with the indicator $\mathcal I$ so that the value function $\hat{V}$ and $V^{\mathcal{E}}$ presenting the expected cumulative failure probability. 


\begin{lemma}
\label{lemma:coverage-of-the-unsafe-actions}
Only a small subspace of the confident action space of expert covers the ground-truth unsafe actions:
$$
  \mathop{\int}_{a \in \mathcal A_\eta(s)} I(s, a)da \le \cfrac{\epsilon}{\eta}.
$$
\end{lemma}

\begin{proof}
According to Assumption~\ref{assumption:expert-failure-rate}, we have:
\begin{equation}
\begin{aligned}
  \epsilon & \ge 
  \mathop{\int}_{a \in \mathcal A} \mathcal{E}(a|s) I(s, a)da 
  = 
  \mathop{\int}_{a \in \mathcal A_\eta(s)} \mathcal{E}(a|s) I(s, a)da +
  \mathop{\int}_{a \notin \mathcal A_\eta(s)} \mathcal{E}(a|s) I(s, a)da.
\end{aligned}
\end{equation}


Following the definition of $\mathcal A_\eta(s)$, we get $\mathcal E(a|s) \ge \eta, \forall a \in \mathcal A_\eta(s)$. Therefore:
\begin{equation}
\begin{aligned}
  \epsilon & \ge 
  \mathop{\int}_{a \in \mathcal A_\eta(s)} \eta I(s, a)da + 0
  =
  \eta \mathop{\int}_{a \in \mathcal A_\eta(s)} I(s, a)da.
\end{aligned}
\end{equation}

Therefore $\mathop{\int}_{a \in \mathcal A_\eta(s)} I(s, a)da \le \cfrac{\epsilon}{\eta}$ is hold.
\end{proof}



\begin{lemma}
\label{lemma:cumulative-probability-of-failure-of-the-expert}
	The cumulative probability of failure of the expert $V^{\mathcal{E}}(s)$ is bounded for all state:
	$$
	V^{\mathcal{E}}(s) \le \cfrac{\epsilon}{1 - \gamma}
	$$
\end{lemma}

\begin{proof}
\begin{equation}
	V^{\mathcal{E}}(s_t) =   
	\expect_{\mathcal{E}}[
		\sum_{t' = t}^{\infty} \gamma^{t' - t}I(s_{t'}, a_{t'})
	]
	=
	\sum_{t' = t}^{\infty}
	\gamma^{t' - t}
	\expect_{\mathcal{E}}[
		 I(s_{t'}, a_{t'})
	]
	\le
	\sum_{t' = t}^{\infty}
	\gamma^{t' - t}
	\epsilon
%	\le
%	\expect_{\mathcal{E}}[
%		\sum_{t' = t}^{\infty} \gamma^{t' - t}\epsilon
%	]
	=
	\cfrac{\epsilon}{1 - \gamma}
\end{equation}
\end{proof}

\textit{\textbf{Theorem.}}
We introduce the main theorem of this work, which shows that the training safety is related to the safety of the expert $\epsilon$ and the confidence level $\eta$.

\begin{theorem}[Upper bound of training risk]
\label{theorem:main}
The expected cumulative probability of failure $\hat{V}$ of the behavior policy $\hat{\pi}$ in EGPO is bounded by the step-wise failure probability of the expert $\epsilon$ as well as the confidence level $\eta$:
$$
\hat{V} 
\le
\cfrac{\epsilon}{1 - \gamma}(
1 + \cfrac{1}{\eta} + \cfrac{\gamma}{1 - \gamma}K'_\eta
),
$$
wherein $
K'_\eta = 
\max_s \mathop{\int}_{a \in \mathcal A_\eta(s)} da
$ is \textbf{negatively correlated} to $\eta$.
\end{theorem}



\begin{proof}

We use the performance difference lemma to show the upper bound. At starting, we first decompose the advantage by splitting the behavior policy:
\begin{equation}
%\begin{aligned}
  \expect_{a\sim \hat{\pi}(\cdot|s)} A^{\mathcal E}(s, a) 
  =
\int_{a \in \mathcal A}
    {\pi}(a|s) \mathbf 1_{a \in \mathcal A_\eta(s)} A^{\mathcal E}(s, a)
    da
+
\int_{a \in \mathcal A} \mathcal{E}(a|s) F(s) A^{\mathcal E}(s, a) da
%\end{aligned}
\end{equation}

The second term is equivalent to $F(s) \expect_{a\sim\mathcal{E}}[ A^{\mathcal E}(s, a)]$, which is equal to zero, according to the definition of advantage.
So we only need to compute the first term.
Firstly we split the integral over whole action space into the confident action space and non-confident action space (which removed by the $\mathbf 1$ operation), then we expand the advantage into detailed form, we have:
\begin{equation}
\begin{aligned}
& \expect_{a\sim \hat{\pi}(\cdot|s)} A^{\mathcal E}(s, a) 
 =   \mathop{\int}_{a \in \mathcal A_\eta(s)} {\pi}(a|s) A^{\mathcal E}(s, a)da ~\\
& = \mathop{\int}_{a \in \mathcal A_\eta(s)} {\pi}(a|s) [
	I(s, a) + \gamma V^{\mathcal{E}}(s') - V^{\mathcal{E}}(s)
	] da ~\\
& =
\underbrace{
\mathop{\int}_{a \in \mathcal A_\eta(s)} {\pi}(a|s) I(s, a)da
}_\text{(a)}
+
\underbrace{
\mathop{\int}_{a \in \mathcal A_\eta(s)} {\pi}(a|s) \gamma V^{\mathcal{E}}(s') da
}_\text{(b)}
-
\underbrace{
\mathop{\int}_{a \in \mathcal A_\eta(s)} {\pi}(a|s) V^{\mathcal{E}}(s) da
}_\text{(c)}
~\\
\end{aligned}
\end{equation}

Following the Lemma~\ref{lemma:coverage-of-the-unsafe-actions}, the term (a) can be bounded as:

\begin{equation}
  \mathop{\int}_{a \in \mathcal A_\eta(s)} {\pi}(a|s) I(s, a)da
  \le
  \mathop{\int}_{a \in \mathcal A_\eta(s)} I(s, a)da
  \le
  \cfrac{\epsilon}{\eta}
\end{equation}

Following the Lemma~\ref{lemma:cumulative-probability-of-failure-of-the-expert}, the term (b) can be written as:

\begin{equation}
  \mathop{\int}_{a \in \mathcal A_\eta(s)} {\pi}(a|s) \gamma V^{\mathcal{E}}(s') da
  \le
  \gamma \mathop{\int}_{a \in \mathcal A_\eta(s)} V^{\mathcal{E}}(s') da
  \le
  \cfrac{\gamma\epsilon}{1 - \gamma} \mathop{\int}_{a \in \mathcal A_\eta(s)} da
  =
  \cfrac{\gamma \epsilon}{1 - \gamma} K_\eta,
\end{equation}
wherein $K_\eta = \mathop{\int}_{a \in \mathcal A_\eta(s)}da$ denoting the area of feasible region in the action space. It is a function related to the expert and $\eta$. If we tighten the guardian by increasing $\eta$, the confident action space determined by the expert $\mathcal A_\eta(s)$ will shrink and the $K_\eta$ will decrease. \textbf{Therefore $K_\eta$ is negatively correlated to $\eta$}.
The term (c) is always non-negative, so after applying the minus to term (c) will make it always $\le 0$.

Aggregating the upper bounds of three terms, we have the bound on the advantage:

\begin{equation}
\label{equation:bound-of-advantage}
\expect_{a\sim \hat{\pi}} A^{\mathcal E}(s, a) 
\le
\cfrac{\epsilon}{\eta}
+
\cfrac{\gamma \epsilon}{1 - \gamma} K_\eta
%\end{aligned}
\end{equation}

Now we put Eq.~\ref{equation:bound-of-advantage} as well as Lemma~\ref{lemma:cumulative-probability-of-failure-of-the-expert} into the performance difference lemma (Lemma~\ref{lemma:performance-difference-lemma}), we have:


\begin{equation}
\begin{aligned}
\hat{V} 
& = 
V^{\mathcal{E}} + 
\cfrac{1}{1-\gamma}
\ \expect_{s\sim P_{\hat{\pi}}} \ 
\expect_{a\sim \hat{\pi}} \ 
[ A^{\mathcal E}(s, a) ]
~\\
& \le
\cfrac{\epsilon}{1 - \gamma}
+
\cfrac{1}{1 - \gamma}
[
\cfrac{\epsilon}{\eta}
+
\cfrac{\gamma \epsilon}{1 - \gamma} K'_\eta
] ~\\
& =
\cfrac{\epsilon}{1 - \gamma}[
1 + \cfrac{1}{\eta} + \cfrac{\gamma}{1 - \gamma}K'_\eta
].
\end{aligned}
\end{equation}


Here we have $
K'_\eta = 
\max_s \mathop{\int}_{a \in \mathcal A_\eta(s)} da
$
.
Now we have proved the upper bound of the discounted probability of failure for the behavior policy in our method.

\end{proof}





